Neural Lander: Stable Drone Landing Control using Learned Dynamics

Precise near-ground trajectory control is difficult for multi-rotor drones, due to the complex aerodynamic effects caused by interactions between multi-rotor airflow and the environment. Conventional control methods often fail to properly account for these complex effects and fall short in accomplishing smooth landing. In this paper, we present a novel deep-learning-based robust nonlinear controller (Neural Lander) that improves control performance of a quadrotor during landing. Our approach combines a nominal dynamics model with a Deep Neural Network (DNN) that learns high-order interactions. We apply spectral normalization (SN) to constrain the Lipschitz constant of the DNN. Leveraging this Lipschitz property, we design a nonlinear feedback linearization controller using the learned model and prove system stability with disturbance rejection. To the best of our knowledge, this is the first DNN-based nonlinear feedback controller with stability guarantees that can utilize arbitrarily large neural nets. Experimental results demonstrate that the proposed controller significantly outperforms a Baseline Nonlinear Tracking Controller in both landing and cross-table trajectory tracking cases. We also empirically show that the DNN generalizes well to unseen data outside the training domain.

==> sections/exp_extra.tex <==
\subsection{Changing DNN Capacity}

To study the influence of the DNN capacity, we trained another two models.  One is 1-layer model, $\hat{\B{f}}_a=\B{A}\B{x}+\B{b}$. The other one is 0-layer model, $\hat{\B{f}}_a=\B{b}$, where we only considered the bias term. The training data and method are same as the 4-layer ReLU DNN in \cref{sec:relu_training}.

\begin{figure}[!t]
\centering
\includegraphics[width=0.4\textwidth, angle=0]{figures/different_models.pdf}
%\vspace{-0.05in}
\caption{Take-off and landing performances with different DNN capacity.}
\vspace{-0.1in}
\label{fig:dnn_capacity}
\end{figure}

The performances of 4-layer, 1-layer, 0-layer models as well as the baseline PD controller are shown in \cref{fig:dnn_capacity}. 

\subsection{Trajectory tracking close to the ground}
In each of the landing scenarios tested, the algorithm tracked a fixed setpoint, ie $p_d = constant, \dot{p_d}=0$.  To validate the performance of the \nn  algorithm, we also tested the performance tracking a non-constant trajectory.  In this case, we chose the desired trajectory to be a circle very near the ground.  

The result were good, see Fig. \ref{fig:ground_comp}.  % TODO: add results
\begin{figure}[!t]
\centering
\includegraphics[width=0.4\textwidth, angle=0]{figures/ground_compare.pdf}
%\vspace{-0.05in}
\caption{\nn{} and the baseline controller performances in the trajectory tracking task. The desired trajectory is a circle close to the ground. Note that the desired heights for \nn{} and PD controller are same.}
\vspace{-0.1in}
\label{fig:ground_comp}
\end{figure}

The comparison of \nn{} and PD controller are shown in \cref{fig:ground_comp}.


